Encode Once, Decode Never: Reusing Audio LM Internals for Efficient Temporal Localization

Audio language models process input audio into rich frame-level representations, but the standard approach to temporal localization generates timestamps as sequences of text tokens, which discards the frame-level representations in favor of autoregressive decoding. However, generating timestamps as tokens is slow and not parallelizable, and tends to hallucinate when producing timestamps outside the training distribution. We propose internal frame-level reuse, a method that trains audio LMs to reuse their own internal audio representations for temporal localization directly, bypassing token generation altogether. We introduce a lightweight prediction head trained via different frame-level objectives: a binary frame classifier and a novel inhomogeneous Poisson process (IHP) loss that models temporal event intensity. Across word localization, speaker diarization, and event localization tasks, our approach can achieve a >50x inference speedup over token-based generation and demonstrates robust length generalization, maintaining high accuracy on out-of-distribution audio durations where token-based models collapse completely. We find that reusing audio frame-level representations yields localization accuracies comparable to (and often better than) finetuned token-based baselines.

==> figures/aux_loss.tex <==
\begin{figure}[ht]
\centering
%\includegraphics[width=\linewidth]{images/sketch/aux_loss.png}
\includegraphics[width=0.7\linewidth]{images/aux_loss.png}
\caption{Generating timestamps with the help of a frame-level auxiliary loss in an audio LLM.}
\label{fig:aux_loss}
\end{figure}

